Searching for Additional Planets in TESS Multi-Planet Systems: Testing Empirical Models Based on Kepler Data

Multi-planet system architectures are frequently used to constrain possible formation and evolutionary pathways of observed exoplanets. Therefore, understanding the predictive and descriptive power of empirical models of these systems is critical to understanding their formation histories. Additionally, if empirical models can reproduce architectures over a range of scales, transit and radial velocity observations can be more easily and effectively used to inform future microlensing, astrometric, and direct imaging surveys. We analyze 52 TESS multi-planet systems previously studied using Dynamite (Dietrich & Apai 2020), who used TESS data alongside empirical models based on Kepler planets to predict additional planets in each system. We analyze additional TESS data to search for these predicted planets. We thereby evaluate the degree to which these models can be used to predict planets in TESS multi-planet systems. Specifically, we study whether a period ratio method or clustered period model is more predictive. We find that the period ratio model predictions are most consistent with the planets discovered since 2020, accounting for detection sensitivity. However, neither model is highly predictive, highlighting the need for additional data and nuanced models to describe the full population. Improved eccentricity and dynamical stability prescriptions incorporated into Dynamite provide a modest improvement in the prediction accuracy. We also find that the current sample of 183 TESS multi-planet systems are are highly dynamically packed, and appear truncated relative to detection biases. These attributes are consistent with the Kepler sample, and suggest a highly efficient formation process.

==> summary_clust.tex <==
\startlongtable
\begin{deluxetable*}{LCC|CC|CC|CCC}
\tablecolumns{10}
\tablefontsize{\scriptsize}
\tablecaption{Summary of the \tnt{} version 1 (v1) and version 3 (v3) predictions under the period ratio model for the 52 TESS multi-planet systems known in 2020. For each version of \tnt{}, the period and radius at the maximum of the posterior probability distributions are reported. We also include the TOIs discovered in these systems since 2020, with associated period and radius reported on ExoFOP. Two of the systems (TOIs 1730 and 1749) have had multiple new planet candidates discovered since 2020, which are shown in separate rows.}
\label{tab:summaryclust}
\tablehead{
    \colhead{TIC} &
    \colhead{TOI} &
    \colhead{Name} &
    \multicolumn{2}{c}{\tnt{} v1} & 
    \multicolumn{2}{c}{\tnt{} v3} & 
    \multicolumn{3}{c}{New TOIs Since 2020} & 
    \colhead{} &
    \colhead{} &
    \colhead{} &
    \colhead{Period (days)} &
    \colhead{Radius ($\mathrm{R_\oplus}$)} &
    \colhead{Period (days)} &
    \colhead{Radius ($\mathrm{R_\oplus}$)} &
    \colhead{TOI} &
    \colhead{Period (days)\tablenotemark{a}} &
    \colhead{Radius ($\mathrm{R_\oplus}$)}}
\startdata
278683844&119&$\mathrm{TOI-119}$&$7.73^{+0.41}_{-0.43}$&$1.91^{+0.66}_{-0.5}$&$3.16^{+0.4}_{-0.5}$&$1.86^{+0.62}_{-0.48}$&&&\\
52368076&125&$\mathrm{TOI-125}$&$6.81^{+0.0}_{-0.56}$&$2.74^{+0.91}_{-0.7}$&$2.55^{+0.4}_{-0.5}$&$2.69^{+0.93}_{-0.69}$&&&\\
425997655&174&$\mathrm{HD~23472}$&$3.12^{+0.0}_{-0.22}$&$1.53^{+1.0}_{-0.6}$&$7.39^{+1.1}_{-1.2}$&$1.27^{+0.45}_{-0.32}$&174.05&$7.91&$0.97 \pm 0.07$\\
307210830&175&$\mathrm{L~98-59}$&$5.22^{+0.03}_{-0.0}$&$1.15^{+0.4}_{-0.3}$&$1.19^{+11.0}_{-6.0}$&$1.12^{+0.38}_{-0.28}$&&&\\
251848941&178&$\mathrm{TOI-178}$&$14.4^{+4.78}_{-0.0}$&$2.67^{+0.89}_{-0.68}$&$3.39^{+0.5}_{-0.7}$&$2.66^{+0.91}_{-0.68}$&178.04&$3.24&$1.51 \pm 1.69$\\
167415965&214&$\mathrm{TOI-214}$&$13.5^{+0.77}_{-1.23}$&$1.46^{+0.87}_{-0.55}$&$5.87^{+0.7}_{-0.9}$&$1.28^{+0.89}_{-0.41}$&214.02&$9.7&$0.81 \pm 0.07$\\
92226327&256&$\mathrm{LHS~ 1140}$&$2.48^{+0.0}_{-0.11}$&$1.45^{+0.5}_{-0.37}$&$2.05^{+0.1}_{-0.2}$&$1.26^{+0.43}_{-0.3}$&&&\\
63898957&261&$\mathrm{TOI-261}$&$4.46^{+0.3}_{-0.0}$&$2.62^{+0.87}_{-0.67}$&$5.36^{+1.55}_{-1.05}$&$2.45^{+0.78}_{-0.62}$&&&\\
164767175&266&$\mathrm{TOI-266}$&$4.93^{+0.0}_{-0.62}$&$2.47^{+0.85}_{-0.64}$&$3.55^{+0.4}_{-0.6}$&$2.41^{+0.81}_{-0.61}$&&&\\
259377017&270&$\mathrm{TOI-270}$&$2.37^{+0.0}_{-0.4}$&$1.86^{+0.64}_{-0.48}$&$1.65^{+0.3}_{-0.4}$&$1.81^{+0.62}_{-0.46}$&&&\\
29781292&282&$\mathrm{HD~28109}$&$42.2^{+0.0}_{-12.0}$&$3.24^{+0.92}_{-0.8}$&$152.4^{+41.7}_{-26.0}$&$3.29^{+1.12}_{-0.85}$&282.04&$22.89&$2.56 \pm 0.34$\\
150030205&286&$\mathrm{TOI-286}$&$5.85^{+0.42}_{-0.0}$&$1.52^{+0.53}_{-0.39}$&$2.84^{+0.2}_{-0.3}$&$1.43^{+0.5}_{-0.36}$&286.02&$39.36&$1.85 \pm 0.14$\\
178155732&396&$\mathrm{HR~858}$&$2.77^{+0.0}_{-0.36}$&$2.16^{+0.75}_{-0.56}$&$2.05^{+0.3}_{-0.4}$&$2.13^{+0.73}_{-0.54}$&396.03&$11.23&$2.08 \pm 0.21$\\
120896927&402&$\mathrm{HD~15337}$&$6.21^{+0.44}_{-0.0}$&$1.88^{+0.65}_{-0.48}$&$3.16^{+0.3}_{-0.2}$&$1.76^{+0.58}_{-0.46}$&&&\\
100990000&411&$\mathrm{HD~22946}$&$3.18^{+0.0}_{-0.22}$&$1.79^{+0.62}_{-0.46}$&$2.55^{+0.2}_{-0.3}$&$1.68^{+0.58}_{-0.44}$&&&\\
31374837&431&$\mathrm{TOI-431}$&$0.64^{+0.04}_{-0.0}$&$1.93^{+1.71}_{-0.8}$&$0.773^{+6.0}_{-3.0}$&$1.49^{+1.59}_{-0.46}$&&&\\
31852980&487&$\mathrm{TOI-487}$&$5.61^{+0.0}_{-0.35}$&$2.43^{+0.83}_{-0.62}$&$4.67^{+0.3}_{-0.4}$&$2.26^{+0.73}_{-0.57}$&&&\\
161477033&553&$\mathrm{TOI-553}$&$54.8^{+3.52}_{-0.0}$&$2.48^{+0.84}_{-0.63}$&$6.74^{+0.9}_{-1.1}$&$2.34^{+0.76}_{-0.59}$&&&\\
377064495&561&$\mathrm{TOI-561}$&$0.59^{+0.05}_{-0.0}$&$1.94^{+0.67}_{-0.5}$&$0.694^{+5.0}_{-2.0}$&$1.89^{+0.64}_{-0.49}$&&&\\
54962195&663&$\mathrm{TOI-663}$&$1.85^{+0.0}_{-0.2}$&$2.12^{+0.73}_{-0.54}$&$1.19^{+0.1}_{-0.2}$&$2.04^{+0.69}_{-0.51}$&663.03&$7.1&$1.99 \pm 0.56$\\
77156829&696&$\mathrm{LHS~ 1678}$&$1.15^{+0.08}_{-0.0}$&$1.1^{+0.39}_{-0.28}$&$1.19^{+0.0}_{-0.0}$&$1.01^{+0.31}_{-0.24}$&696.03&$4.97&$0.86 \pm 2.66$\\
149302744&699&$\mathrm{TOI-699}$&$11.4^{+0.0}_{-0.74}$&$2.36^{+0.8}_{-0.61}$&$9.29^{+0.6}_{-0.8}$&$2.19^{+0.735}_{-0.545}$&699.03&$672.64 \pm 0.01$&$2.97 \pm 1.86$\\
150428135&700&$\mathrm{TOI-700}$&$23.0^{+4.17}_{-0.0}$&$1.57^{+1.11}_{-0.64}$&$4.89^{+0.8}_{-1.0}$&$1.21^{+1.1}_{-0.37}$&700.04&$27.81&$0.95 \pm 0.31$\\
237928815&703&$\mathrm{TOI-703}$&$6.48^{+0.0}_{-0.4}$&$2.65^{+0.88}_{-0.68}$&$4.89^{+0.4}_{-0.4}$&$2.43^{+0.79}_{-0.61}$&&&\\
150151262&712&$\mathrm{TOI-712}$&$74.5^{+15.0}_{-0.0}$&$3.24^{+0.92}_{-0.79}$&$26.7^{+3.2}_{-4.2}$&$3.24^{+1.08}_{-0.82}$&712.04&$84.84&$2.04 \pm 0.23$\\
167600516&713&$\mathrm{TOI-713}$&$1.42^{+0.0}_{-0.1}$&$1.67^{+1.19}_{-0.7}$&$1.19^{+0.1}_{-0.1}$&$1.25^{+1.14}_{-0.37}$&&&\\
219195044&714&$\mathrm{TOI-714}$&$14.8^{+0.77}_{-0.0}$&$3.24^{+0.92}_{-0.8}$&$2.28^{+0.1}_{-0.2}$&$2.96^{+0.93}_{-0.72}$&&&\\
36724087&732&$\mathrm{LTT~3780}$&$1.06^{+0.06}_{-0.0}$&$1.28^{+0.45}_{-0.33}$&$1.19^{+9.0}_{-7.0}$&$1.18^{+0.39}_{-0.28}$&&&\\
181804752&736&$\mathrm{LP~791-18}$&$1.5^{+0.07}_{-0.0}$&$1.6^{+1.14}_{-0.66}$&$1.65^{+0.1}_{-0.2}$&$1.08^{+0.69}_{-0.28}$&&&\\
178819686&763&$\mathrm{TOI-763}$&$4.19^{+0.0}_{-0.26}$&$3.25^{+0.91}_{-0.8}$&$3.16^{+0.3}_{-0.272}$&$3.05^{+0.98}_{-0.75}$&&&\\
306996324&776&$\mathrm{TOI-776}$&$11.4^{+0.0}_{-0.19}$&$1.77^{+0.61}_{-0.46}$&$4.46^{+0.6}_{-0.6}$&$1.7^{+0.57}_{-0.44}$&&&\\
271596225&797&$\mathrm{TOI-797}$&$2.44^{+0.16}_{-0.0}$&$1.34^{+0.46}_{-0.34}$&$1.07^{+0.1}_{-0.1}$&$1.2^{+0.4}_{-0.3}$&797.03&$2.73&$1.02 \pm 1.82$\\
440887364&836&$\mathrm{TOI-836}$&$5.15^{+0.33}_{-0.0}$&$2.07^{+0.72}_{-0.53}$&$2.28^{+0.2}_{-0.2}$&$1.92^{+0.63}_{-0.5}$&&&\\
79748331&1064&$\mathrm{TOI-1064}$&$8.91^{+0.0}_{-0.08}$&$2.78^{+0.91}_{-0.71}$&$3.39^{+0.4}_{-0.5}$&$2.69^{+0.9}_{-0.68}$&&&\\
142276270&1136&$\mathrm{TOI-1136}$&$9.15^{+0.0}_{-0.72}$&$3.47^{+0.89}_{-0.83}$&$3.55^{+0.6}_{-0.9}$&$3.07^{+1.04}_{-0.79}$&1136.04&$18.8&$2.16 \pm 0.88$\\
260647166&1233&$\mathrm{HD~108236}$&$9.58^{+1.11}_{-1.43}$&$1.9^{+0.66}_{-0.49}$&$9.29^{+3.1}_{-22.6}$&$1.87^{+0.65}_{-0.48}$&&&\\
153951307&1238&$\mathrm{TOI-1238}$&$1.02^{+0.07}_{-0.0}$&$1.72^{+1.04}_{-0.65}$&$1.19^{+0.1}_{-0.0}$&$1.37^{+0.96}_{-0.41}$&&&\\
230127302&1246&$\mathrm{TOI-1246}$&$13.9^{+0.0}_{-0.83}$&$2.9^{+0.92}_{-0.73}$&$10.2^{+1.0}_{-0.7}$&$2.91^{+0.96}_{-0.73}$&1246.04&$37.93&$3.24 \pm 1.18$\\
355867695&1260&$\mathrm{TOI-1260}$&$4.32^{+0.26}_{-0.0}$&$2.53^{+0.85}_{-0.65}$&$1.65^{+0.1}_{-0.1}$&$2.32^{+0.746}_{-0.59}$&1260.03&$49.83&$3.83 \pm 0.48$\\
467179528&1266&$\mathrm{TOI-1266}$&$26.4^{+3.35}_{-0.0}$&$1.92^{+0.66}_{-0.49}$&$5.36^{+0.6}_{-0.8}$&$1.84^{+0.61}_{-0.47}$&&&\\
198241702&1269&$\mathrm{TOI-1269}$&$3.2^{+0.0}_{-0.2}$&$2.46^{+0.83}_{-0.63}$&$2.28^{+0.2}_{-0.2}$&$2.27^{+0.74}_{-0.57}$&1269.02&$9.24&$2.23 \pm 0.15$\\
153949511&1277&$\mathrm{TOI-1277}$&$19.9^{+1.28}_{-0.0}$&$3.26^{+0.91}_{-0.8}$&&&&&\\
269701147&1339&$\mathrm{HD~191939}$&$18.8^{+0.0}_{-3.16}$&$2.26^{+1.37}_{-0.83}$&$15.4^{+1.1}_{-1.0}$&$2.09^{+1.45}_{-0.71}$&&&\\
219852882&1346&$\mathrm{TOI-1346}$&$1.33^{+0.0}_{-0.09}$&$2.01^{+0.7}_{-0.52}$&$1.07^{+0.0}_{-0.1}$&$1.88^{+0.62}_{-0.49}$&1346.02&$1.76&$2.52 \pm 0.28$\\
229650439&1438&$\mathrm{TOI-1438}$&$7.04^{+0.02}_{-0.15}$&$2.53^{+0.85}_{-0.65}$&$2.55^{+0.3}_{-0.4}$&$2.44^{+0.83}_{-0.61}$&1438.02&$9.43&$2.37 \pm 0.17$\\
356158613&1449&$\mathrm{TOI-1449}$&$3.28^{+0.2}_{-0.0}$&$2.0^{+2.17}_{-0.67}$&&&&&\\
198390247&1453&$\mathrm{TOI-1453}$&$3.32^{+0.0}_{-0.45}$&$1.67^{+1.08}_{-0.65}$&$2.28^{+0.3}_{-0.4}$&$1.47^{+1.1}_{-0.5}$&1453.02&$4.31&$1.13 \pm 0.09$\\
243185500&1468&$\mathrm{TOI-1468}$&$2.68^{+0.15}_{-0.0}$&$1.63^{+0.57}_{-0.42}$&$3.16^{+0.4}_{-5.4}$&$1.49^{+0.52}_{-0.37}$&&&\\
283722336&1469&$\mathrm{HD~219134}$&$5.21^{+0.0}_{-0.35}$&$1.55^{+0.54}_{-0.4}$&$1.84^{+0.2}_{-0.2}$&$1.44^{+0.5}_{-0.36}$&&&\\
130181866&1726&$\mathrm{HD~63433}$&$9.34^{+0.63}_{-0.0}$&$2.36^{+0.81}_{-0.6}$&$4.46^{+0.3}_{-0.4}$&$2.19^{+0.72}_{-0.55}$&1726.02&$20.54&$2.57 \pm 0.3$\\
130181866&&&$9.34^{+0.63}_{-0.0}$&$2.36^{+0.81}_{-0.6}$&$4.46^{+0.3}_{-0.4}$&$2.19^{+0.72}_{-0.55}$&1726.01&$7.11&$2.24 \pm 0.15$\\
318022259&1730&$\mathrm{TOI-1730}$&$1.58^{+0.0}_{-0.1}$&$1.63^{+0.57}_{-0.42}$&$1.19^{+0.1}_{-0.1}$&$1.49^{+0.52}_{-0.37}$&1730.02&$2.16&$1.48 \pm 0.11$\\
318022259&&&$1.58^{+0.0}_{-0.1}$&$1.63^{+0.57}_{-0.42}$&$1.19^{+0.1}_{-0.1}$&$1.49^{+0.52}_{-0.37}$&1730.01&$6.23&$2.76 \pm 0.96$\\
318022259&&&$1.58^{+0.0}_{-0.1}$&$1.63^{+0.57}_{-0.42}$&$1.19^{+0.1}_{-0.1}$&$1.49^{+0.52}_{-0.37}$&1730.03&$12.57&$2.44 \pm 0.11$\\
233602827&1749&$\mathrm{TOI-1749}$&$6.25^{+0.2}_{-0.0}$&$2.27^{+0.78}_{-0.58}$&$2.55^{+0.2}_{-0.2}$&$2.08^{+0.67}_{-0.51}$&1749.03&$2.39&$1.34 \pm 2.03$\\
233602827&&&$6.25^{+0.2}_{-0.0}$&$2.27^{+0.78}_{-0.58}$&$2.55^{+0.2}_{-0.2}$&$2.08^{+0.67}_{-0.51}$&1749.02&$9.04&$2.25 \pm 1.36$\\
233602827&&&$6.25^{+0.2}_{-0.0}$&$2.27^{+0.78}_{-0.58}$&$2.55^{+0.2}_{-0.2}$&$2.08^{+0.67}_{-0.51}$&1749.01&$4.49&$2.0 \pm 1.01$&
\enddata
\tablenotetext{a}{Typical errors on the period of TOIs reported on ExoFOP are $<0.001$.}
\end{deluxetable*}


==> summary_ratio.tex <==
\startlongtable
\begin{deluxetable*}{LCC|CC|CC|CCC}
\tablecolumns{10}
\tablefontsize{\scriptsize}
\tablecaption{Summary of the \tnt{} version 1 (v1) and version 3 (v3) predictions under the period ratio model for the 52 TESS multi-planet systems known in 2020. For each version of \tnt{}, the period and radius at the maximum of the posterior probability distributions are reported. We also include the TOIs discovered in these systems since 2020, with associated period and radius reported on ExoFOP. Two of the systems (TOIs 1730 and 1749) have had multiple new planet candidates discovered since 2020, which are shown in separate rows.}
\label{tab:summaryratio}
\tablehead{
    \colhead{TIC} &
    \colhead{TOI} &
    \colhead{Name} &
    \multicolumn{2}{c}{\tnt{} v1} & 
    \multicolumn{2}{c}{\tnt{} v3} & 
    \multicolumn{3}{c}{New TOIs Since 2020} & 
    \colhead{} &
    \colhead{} &
    \colhead{} &
    \colhead{Period (days)} &
    \colhead{Radius ($\mathrm{R_\oplus}$)} &
    \colhead{Period (days)} &
    \colhead{Radius ($\mathrm{R_\oplus}$)} &
    \colhead{TOI} &
    \colhead{Period (days)\tablenotemark{a}} &
    \colhead{Radius ($\mathrm{R_\oplus}$)}}
\startdata
278683844&119&$\mathrm{TOI-119}$&$19.7^{+7.96}_{-3.62}$&$1.91^{+0.66}_{-0.49}$&$20.3^{+9.6}_{-5.7}$&$1.91^{+0.66}_{-0.49}$&&&\\
52368076&125&$\mathrm{TOI-125}$&$36.8^{+14.9}_{-6.77}$&$2.75^{+0.9}_{-0.7}$&$38.5^{+14.8}_{-8.6}$&$2.77^{+0.95}_{-0.71}$&&&\\
425997655&174&$\mathrm{HD~23472}$&$6.95^{+1.14}_{-0.98}$&$1.29^{+0.45}_{-0.33}$&$7.39^{+0.9}_{-0.9}$&$1.28^{+0.45}_{-0.32}$&174.05&$7.91 &$0.97 \pm 0.07$\\
307210830&175&$\mathrm{L~98-59}$&$13.7^{+5.55}_{-2.52}$&$1.15^{+0.4}_{-0.3}$&$15.4^{+6.5}_{-3.7}$&$1.15^{+0.4}_{-0.29}$&&&\\
251848941&178&$\mathrm{TOI-178}$&$19.1^{+7.71}_{-3.51}$&$2.67^{+0.88}_{-0.68}$&$20.3^{+8.3}_{-5.1}$&$2.68^{+0.93}_{-0.68}$&178.04&$3.24 &$1.51 \pm 1.69$\\
167415965&214&$\mathrm{TOI-214}$&$34.2^{+13.8}_{-6.28}$&$1.46^{+0.88}_{-0.54}$&$36.8^{+14.4}_{-8.4}$&$1.44^{+0.88}_{-0.52}$&214.02&$9.70 &$0.81 \pm 0.07$\\
92226327&256&$\mathrm{LHS~1140}$&$9.81^{+4.03}_{-3.05}$&$1.45^{+0.5}_{-0.37}$&$9.29^{+2.0}_{-1.7}$&$1.43^{+0.5}_{-0.36}$&&&\\
63898957&261&$\mathrm{TOI-261}$&$6.62^{+1.51}_{-1.23}$&$2.62^{+0.87}_{-0.67}$&$6.44^{+0.7}_{-0.6}$&$2.63^{+0.91}_{-0.68}$&&&\\
164767175&266&$\mathrm{TOI-266}$&$19.8^{+8.0}_{-3.64}$&$2.48^{+0.85}_{-0.64}$&$21.2^{+9.4}_{-5.8}$&$2.48^{+0.86}_{-0.64}$&&&\\
259377017&270&$\mathrm{TOI-270}$&$21.0^{+8.47}_{-3.85}$&$1.86^{+0.65}_{-0.48}$&$23.2^{+9.0}_{-5.6}$&$1.85^{+0.65}_{-0.47}$&&&\\
29781292&282&$\mathrm{HD~28109}$&$12.0^{+5.38}_{-3.23}$&$3.25^{+0.91}_{-0.8}$&$11.7^{+1.8}_{-2.4}$&$3.34^{+1.14}_{-0.86}$&282.04&$22.89 &$2.56 \pm 0.34$\\
150030205&286&$\mathrm{TOI-286}$&$13.6^{+7.94}_{-5.35}$&$1.52^{+0.53}_{-0.39}$&$80.2^{+32.5}_{-30.8}$&$1.52^{+0.53}_{-0.39}$&286.02&$39.36 &$1.85 \pm 0.14$\\
178155732&396&$\mathrm{HR~858}$&$11.0^{+4.45}_{-2.02}$&$2.16^{+0.75}_{-0.56}$&$21.2^{+8.9}_{-5.6}$&$2.16^{+0.75}_{-0.55}$&396.03&$11.23 &$2.08 \pm 0.21$\\
120896927&402&$\mathrm{HD~15337}$&$9.04^{+1.87}_{-1.55}$&$1.88^{+0.65}_{-0.49}$&$9.29^{+0.9}_{-0.9}$&$1.87^{+0.66}_{-0.48}$&&&\\
100990000&411&$\mathrm{HD~22946}$&$17.6^{+7.13}_{-3.24}$&$1.79^{+0.62}_{-0.46}$&$18.5^{+8.3}_{-5.1}$&$1.79^{+0.62}_{-0.46}$&&&\\
31374837&431&$\mathrm{TOI-431}$&$23.0^{+9.28}_{-4.22}$&$1.93^{+1.71}_{-0.81}$&$26.7^{+11.0}_{-6.8}$&$2.03^{+1.77}_{-0.89}$&&&\\
31852980&487&$\mathrm{TOI-487}$&$13.7^{+2.23}_{-2.3}$&$2.43^{+0.82}_{-0.62}$&$12.8^{+1.1}_{-1.0}$&$2.43^{+0.83}_{-0.63}$&&&\\
161477033&553&$\mathrm{TOI-553}$&$75.3^{+30.5}_{-13.9}$&$2.48^{+0.84}_{-0.64}$&$23.2^{+1.6}_{-1.6}$&$2.48^{+0.85}_{-0.64}$&&&\\
377064495&561&$\mathrm{TOI-561}$&$30.0^{+12.1}_{-5.52}$&$1.94^{+0.68}_{-0.5}$&$29.2^{+12.9}_{-7.8}$&$1.93^{+0.67}_{-0.49}$&&&\\
54962195&663&$\mathrm{TOI-663}$&$8.66^{+3.5}_{-1.59}$&$2.11^{+0.73}_{-0.55}$&$9.29^{+4.2}_{-2.5}$&$2.12^{+0.73}_{-0.55}$&663.03&$7.10 &$1.99 \pm 0.56$\\
77156829&696&$\mathrm{LHS~1678}$&$27.2^{+11.0}_{-5.0}$&$1.1^{+0.38}_{-0.28}$&$29.2^{+12.1}_{-7.6}$&$1.1^{+0.38}_{-0.28}$&696.03&$4.97 &$0.86 \pm 2.66$\\
149302744&699&$\mathrm{TOI-699}$&$62.0^{+25.0}_{-11.4}$&$2.36^{+0.8}_{-0.6}$&$7.39^{+1.2}_{-1.6}$&$2.35^{+0.82}_{-0.6}$&699.03&$672.64 $&$2.97 \pm 1.86$\\
150428135&700&$\mathrm{TOI-700}$&$68.9^{+27.9}_{-12.7}$&$1.59^{+1.1}_{-0.66}$&$73.2^{+29.5}_{-27.1}$&$1.52^{+1.13}_{-0.6}$&700.04&$27.81 &$0.95 \pm 0.31$\\
237928815&703&$\mathrm{TOI-703}$&$19.8^{+6.44}_{-4.86}$&$2.64^{+0.88}_{-0.67}$&$20.3^{+3.4}_{-3.1}$&$2.62^{+0.9}_{-0.66}$&&&\\
150151262&712&$\mathrm{TOI-712}$&$22.3^{+7.51}_{-5.77}$&$3.24^{+0.92}_{-0.8}$&$21.2^{+4.1}_{-3.6}$&$3.32^{+1.14}_{-0.85}$&712.04&$84.84 &$2.04 \pm 0.23$\\
167600516&713&$\mathrm{TOI-713}$&$14.4^{+8.81}_{-11.5}$&$1.66^{+1.22}_{-0.68}$&$73.2^{+29.1}_{-29.2}$&$1.62^{+1.24}_{-0.66}$&&&\\
219195044&714&$\mathrm{TOI-714}$&$18.7^{+7.58}_{-3.45}$&$3.25^{+0.92}_{-0.8}$&$23.2^{+9.9}_{-5.8}$&$3.34^{+1.15}_{-0.86}$&&&\\
36724087&732&$\mathrm{LTT~3780}$&$22.6^{+9.13}_{-4.15}$&$1.29^{+0.45}_{-0.33}$&$26.7^{+10.6}_{-6.5}$&$1.28^{+0.45}_{-0.33}$&&&\\
181804752&736&$\mathrm{LP~791-18}$&$2.18^{+0.72}_{-0.54}$&$1.61^{+1.14}_{-0.66}$&$1.84^{+0.3}_{-0.2}$&$1.56^{+1.16}_{-0.62}$&&&\\
178819686&763&$\mathrm{TOI-763}$&$22.6^{+9.14}_{-4.16}$&$3.24^{+0.92}_{-0.8}$&$26.7^{+11.0}_{-6.8}$&$3.34^{+1.15}_{-0.86}$&&&\\
306996324&776&$\mathrm{TOI-776}$&$28.8^{+11.7}_{-5.3}$&$1.77^{+0.61}_{-0.46}$&$33.6^{+12.2}_{-7.6}$&$1.74^{+0.61}_{-0.44}$&&&\\
271596225&797&$\mathrm{TOI-797}$&$2.73^{+0.29}_{-0.27}$&$1.34^{+0.46}_{-0.34}$&$9.29^{+3.2}_{-2.1}$&$1.34^{+0.46}_{-0.35}$&797.03&$2.73 &$1.02 \pm 1.82$\\
440887364&836&$\mathrm{TOI-836}$&$15.8^{+6.4}_{-2.91}$&$2.08^{+0.72}_{-0.53}$&$18.5^{+7.5}_{-4.6}$&$2.07^{+0.73}_{-0.53}$&&&\\
79748331&1064&$\mathrm{TOI-1064}$&$22.5^{+9.11}_{-4.14}$&$2.77^{+0.91}_{-0.71}$&$26.7^{+11.1}_{-6.6}$&$2.79^{+0.97}_{-0.72}$&&&\\
142276270&1136&$\mathrm{TOI-1136}$&$48.5^{+19.6}_{-8.91}$&$3.47^{+0.88}_{-0.83}$&$50.7^{+25.3}_{-11.3}$&$3.09^{+1.06}_{-0.79}$&1136.04&$18.80 &$2.16 \pm 0.88$\\
260647166&1233&$\mathrm{HD~108236}$&$9.38^{+1.0}_{-0.91}$&$1.89^{+0.66}_{-0.49}$&$36.8^{+14.3}_{-8.5}$&$1.9^{+0.65}_{-0.49}$&&&\\
153951307&1238&$\mathrm{TOI-1238}$&$6.07^{+2.45}_{-1.12}$&$1.71^{+1.04}_{-0.64}$&$1.48^{+0.2}_{-0.2}$&$1.71^{+1.04}_{-0.64}$&&&\\
230127302&1246&$\mathrm{TOI-1246}$&$10.4^{+1.93}_{-1.43}$&$2.91^{+0.92}_{-0.74}$&$10.2^{+0.9}_{-0.9}$&$3.01^{+1.05}_{-0.77}$&1246.04&$37.93 &$3.24 \pm 1.18$\\
355867695&1260&$\mathrm{TOI-1260}$&$13.8^{+5.58}_{-2.54}$&$2.53^{+0.85}_{-0.65}$&$15.4^{+5.9}_{-3.9}$&$2.53^{+0.87}_{-0.65}$&1260.03&$49.83 &$3.83 \pm 0.48$\\
467179528&1266&$\mathrm{TOI-1266}$&$34.6^{+14.0}_{-6.37}$&$1.92^{+0.66}_{-0.49}$&$36.8^{+13.6}_{-8.3}$&$1.91^{+0.66}_{-0.49}$&&&\\
198241702&1269&$\mathrm{TOI-1269}$&$17.0^{+6.88}_{-3.13}$&$2.45^{+0.83}_{-0.63}$&$18.5^{+7.7}_{-4.8}$&$2.46^{+0.84}_{-0.63}$&1269.02&$9.24 &$2.23 \pm 0.15$\\
153949511&1277&$\mathrm{TOI-1277}$&$68.3^{+27.6}_{-12.6}$&$3.26^{+0.92}_{-0.8}$&&&&&\\
269701147&1339&$\mathrm{HD~191939}$&$52.6^{+21.3}_{-9.68}$&$2.26^{+1.37}_{-0.83}$&$14.7^{+1.0}_{-0.8}$&$2.29^{+1.46}_{-0.85}$&&&\\
219852882&1346&$\mathrm{TOI-1346}$&$3.13^{+0.51}_{-0.47}$&$2.01^{+0.7}_{-0.52}$&$3.16^{+0.2}_{-0.3}$&$2.01^{+0.7}_{-0.52}$&1346.02&$1.76 &$2.52 \pm 0.28$\\
229650439&1438&$\mathrm{TOI-1438}$&$17.4^{+7.02}_{-3.19}$&$2.53^{+0.85}_{-0.65}$&$18.5^{+8.2}_{-5.0}$&$2.53^{+0.87}_{-0.65}$&1438.02&$9.43 &$2.37 \pm 0.17$\\
356158613&1449&$\mathrm{TOI-1449}$&$7.49^{+6.07}_{-3.17}$&$1.99^{+2.18}_{-0.67}$&&&&&\\
198390247&1453&$\mathrm{TOI-1453}$&$12.1^{+4.91}_{-2.23}$&$1.67^{+1.08}_{-0.66}$&$13.4^{+6.2}_{-3.6}$&$1.65^{+1.08}_{-0.64}$&1453.02&$4.31 &$1.13 \pm 0.09$\\
243185500&1468&$\mathrm{TOI-1468}$&$3.82^{+0.93}_{-0.75}$&$1.63^{+0.57}_{-0.42}$&$33.6^{+12.8}_{-7.9}$&$1.63^{+0.56}_{-0.42}$&&&\\
283722336&1469&$\mathrm{HD~219134}$&$12.5^{+5.04}_{-2.29}$&$1.55^{+0.54}_{-0.4}$&$12.8^{+5.7}_{-3.6}$&$1.55^{+0.54}_{-0.4}$&&&\\
130181866&1726&$\mathrm{HD~63433}$&$12.1^{+1.84}_{-1.6}$&$2.36^{+0.8}_{-0.61}$&$42.2^{+16.1}_{-9.2}$&$2.35^{+0.81}_{-0.6}$&1726.02&$20.54 &$2.57 \pm 0.3$\\
130181866&1726&$\mathrm{HD~63433}$&$12.1^{+1.84}_{-1.6}$&$2.36^{+0.8}_{-0.61}$&$42.2^{+16.1}_{-9.2}$&$2.35^{+0.81}_{-0.6}$&1726.01&$7.11 &$2.24 \pm 0.15$\\
318022259&1730&$\mathrm{TOI-1730}$&$3.66^{+0.56}_{-0.48}$&$1.64^{+0.57}_{-0.42}$&$12.8^{+5.4}_{-3.3}$&$1.63^{+0.57}_{-0.42}$&1730.02&$2.16 &$1.48 \pm 0.11$\\
318022259&&&$3.66^{+0.56}_{-0.48}$&$1.64^{+0.57}_{-0.42}$&$12.8^{+5.4}_{-3.3}$&$1.63^{+0.57}_{-0.42}$&1730.01&$6.23 &$2.76 \pm 0.96$\\
318022259&&&$3.66^{+0.56}_{-0.48}$&$1.64^{+0.57}_{-0.42}$&$12.8^{+5.4}_{-3.3}$&$1.63^{+0.57}_{-0.42}$&1730.03&$12.57 &$2.44 \pm 0.11$\\
233602827&1749&$\mathrm{TOI-1749}$&$16.7^{+6.74}_{-3.06}$&$2.27^{+0.78}_{-0.59}$&$20.3^{+7.7}_{-4.8}$&$2.26^{+0.79}_{-0.58}$&1749.03&$2.39 &$1.34 \pm 2.03$\\
233602827&&$&$16.7^{+6.74}_{-3.06}$&$2.27^{+0.78}_{-0.59}$&$20.3^{+7.7}_{-4.8}$&$2.26^{+0.79}_{-0.58}$&1749.02&$9.04 &$2.25 \pm 1.36$\\
233602827&&$&$16.7^{+6.74}_{-3.06}$&$2.27^{+0.78}_{-0.59}$&$20.3^{+7.7}_{-4.8}$&$2.26^{+0.79}_{-0.58}$&1749.01&$4.49 &$2.0 \pm 1.01$\\
\enddata
\tablenotetext{a}{Typical errors on the period of TOIs reported on ExoFOP are $<0.001$.}
\end{deluxetable*}

